SAPPHIRE: Approaches for Enhanced Concept-to-Text Generation

We motivate and propose a suite of simple but effective improvements for concept-to-text generation called SAPPHIRE: Set Augmentation and Post-hoc PHrase Infilling and REcombination. We demonstrate their effectiveness on generative commonsense reasoning, a.k.a. the CommonGen task, through experiments using both BART and T5 models. Through extensive automatic and human evaluation, we show that SAPPHIRE noticeably improves model performance. An in-depth qualitative analysis illustrates that SAPPHIRE effectively addresses many issues of the baseline model generations, including lack of commonsense, insufficient specificity, and poor fluency.

==> sections/camreadytodos.tex <==
-Original test split results (CommonGen authors) [AWAITING REPLY]
-Code (clean) and data release



DONE:
-Reference for Pitman test
-Add references for metrics (e.g. BLEU, ROUGE, SPICE, CIDEr, METEOR, etc.)
-Expand related works section
-Add data aug survey paper reference (and maybe some others like GenAug) in future work and related works
-Create GitHub repo and add link
-Cam-ready style stuff and author list
-Bring back more examples in the tables
-Claims too strong
-Clarify that we don't use human examples for inference
-Qualitative examples
-Address reviewer comments
-Move tables to more appropriate pages
-Remove vspace hacks and make spacing look nicer
-Fix/redo statistical significance
-Add acknowledgements (Graham, Divyansh, Ritam)
-More hyperparameter results tables/graphs (e.g. for 1-5 keywords)
-Double check references (cite published versions)

FORGET IT:
-More training details like best epochs chosen per model in appendices
-Model diagram on first page
-Enlarge qualitative example tables (maybe)
